On the Complexity of Finding a Diverse and Representative Committee using a Monotone, Separable Positional Multiwinner Voting Rule

Fairness in multiwinner elections, a growing line of research in computational social choice, primarily concerns the use of constraints to ensure fairness. Recent work proposed a model to find a diverse \emph{and} representative committee and studied the model's computational aspects. However, the work gave complexity results under major assumptions on how the candidates and the voters are grouped. Here, we close this gap and classify the complexity of finding a diverse and representative committee using a monotone, separable positional multiwinner voting rule, conditioned \emph{only} on the assumption that P $\neq$ NP.

==> new_tex/model.tex <==
\section{Fair Allocation Model}
\label{sec:Model}

In this section, we formally define a model that maps the \DIRE Committee Winner Determination problem to a problem of fairly allocating indivisible goods. The model mitigates unfairness to the voter population caused by \DIRE Committees. We first define constraints. 

\paragraph{Diversity Constraints,} denoted by $l^D_G \in [1,$ $\min(k, |G|)]$ %\ideally will be better if it is min(k, |G|)
for each candidate group $G \in \mathcal{G}$, enforces at least $l^D_G$ candidates from the group $G$ to be in the committee $W$. Formally,  $\forall$ $G \in \mathcal{G}$, $|G \cap W|\geq l^D_G$. 
%\julia{What's $D$ and why do you need it?  R is also a voting rule.  I wouldn't use D or R; attributes are attributes, if it's for candidates - you call that diversity, if it's for voters - you call that representation.}\kunal{I'll remove it from the attributes. But, we will need it to identify the 2 different types of constraints. I'll change the notation for scoring rule.} \julia{Too late to change now probably, but this is very non-standard notation. What you have here are categorical attributes; each categorical attribute has a cardinality (the number of values); each attribute partitions the candidates or the voters.}
%We note that we do not propose to use the upper bounds as it induces quota system, which is not desirable from social choice perspective. 

%\vspace{-0.15cm}
\paragraph{Representation Constraints,} denoted by $l^R_P \in [1,k]$ for each voter population $P \in \mathcal{P}$, enforces at least $l^R_P$ candidates from the population $P$'s committee $W_P$ to be in the committee $W$. Formally,  $\forall$ $P \in \mathcal{P}$, $|W_P \cap W|\geq l^R_P$.

\begin{definition}
\label{def-DiReCWD}
\textbf{\DIRE Committee Winner Determination (\DiReCWD):}  We are given an instance of election $E=(C,V)$,  
%set $C$ of $m$ candidates, a set $V$ of $n$ voters such that each voter $v \in V$ has a preference list $\succ_{v}$ over $m$ candidates, 
a committee size $k \in [m]$, a set of candidate groups $\mathcal{G}$ under $\mu$ attributes and their diversity constraints $l^D_G$  $\forall$ $G \in \mathcal{G}$, a set of voter populations $\mathcal{P}$ under $\pi$ attributes and their representation constraints $l^R_P$ and the winning committees $W_P$  $\forall$ $P \in \mathcal{P}$, and a \csr $\mathtt{f}$.
Let $\mathcal{W}$ denote the family of all size-$k$ committees. 
The goal of \DiReCWD is to select committees $W \in \mathcal{W}$ that satisfy  diversity and representation constraints such that $|G\cap W|\geq l^D_G$  $\forall$ $G\in \mathcal{G}$ and $|W_P\cap W|\geq l^R_P$  $\forall$ $P\in \mathcal{P}$ and maximizes, $\forall W \in \mathcal{W}$, $\mathtt{f}(W)$. Committees that satisfy the constraints are \DiRe committees.
\end{definition}


Example~\ref{eg-balanced} showed that a \DiRe committee may create or propagate biases by systematically increasing the selection of lower preferred candidates. This may result in more loss in utility to historically disadvantaged, smaller voter populations.

To mitigate this, we model our problem of selecting a committee as allocating goods (candidates) into $k$ slots. Hence, to assess the quality of candidates being selected from voter populations, we borrow ideas from the literature on the problem of fair resource allocation of indivisible goods \cite{brandt2016handbook}. Formally, given a set of $n$ agents, a set of $m$ resources, and a valuation each agent gives to each resource, the problem of fair allocation is to partition the resources among agents such that the allocation is fair. There are three classic fairness desiderata, namely, proportionality, envy-freeness, and equitability \cite{freemanrecent}. Intuitively, proportionality requires that each agent should receive her ``fair share'' of the utility, envy-freeness requires no agent should wish to swap her allocation with another agent, and equitability requires all agents should have the exact same value for their allocations and no agent should be jealous of what another agent receives. As balancing the loss in utility to candidate groups is analogous to balancing the fairness in ranking \cite{yang2019balanced}, we focus on balancing the loss in utility to voter populations. We propose varying notions of envyfreeness to balance the loss in utility to voter populations\footnote{Our model, \emph{Fairly Allocating} Utility in Constrained Multiwinner Elections, is analogous to a Swiss Army knife. The model can be applicable to more or less any context of a constrained multiwinner election and the setting of the model can be chosen based on the context.}:

\begin{table*}[t]
\centering
\begin{tabular}{l|l||c|c||c|c||c|c|c||c|c|c}
\toprule
 & Committee & score & DiRe & \multicolumn{2}{c||}{FEC} & \multicolumn{3}{c||}{UEC} & \multicolumn{3}{c}{WEC}\\
& &  & Committee & \multicolumn{2}{c||}{up to} & \multicolumn{3}{c||}{up to} & \multicolumn{3}{c}{up to}\\
 \cline{5-12}
&  &  &  & 0 & 1 & 0 & 1 & 2 & 0 & $\frac{1}{13}$& $\frac{2}{13}$\\
\midrule
1&$\{c_1, c_2, c_6, c_5\}$&342& \xmark &\cmark&\cmark&\cmark&\cmark&\cmark&\cmark&\cmark&\cmark\\
\hline

2&$\{c_1, c_6, c_3, c_8\}$&286& \cmark &\xmark&\cmark&\xmark&\xmark&\cmark&\xmark&\xmark&\cmark\\
\hline

3&$\{c_1, c_5, c_3, c_8\}$&285& \cmark &\cmark&\cmark&\cmark&\cmark&\cmark&\xmark&\cmark&\cmark\\
\hline

4&$\{c_1, c_5, c_3, c_7\}$&284& \cmark &\cmark&\cmark&\xmark&\xmark&\cmark&\cmark&\cmark&\cmark\\

\bottomrule
\end{tabular}
%}
\caption{Properties satisfied by various example committees selected using the election setup given in Figure~\ref{fig:whatexample/candidates} and Figure~\ref{fig:whatexample/voters}. Each row corresponds to a committee being (row 1) optimal, (row 2) optimal DiRe, (row 3) optimal FEC and optimal UEC given it is DiRe, and (row 4) optimal WEC given it is DiRe. `DiRe' denotes a committee satisfying diversity and representation constraints. `FEC' denotes Favorite-Envyfree-Committee. `UEC' denotes Utility-Envyfree-Committee. `WEC' denotes Weighted-Envyfree-Committee.}

\label{tab:FECUECWEC-examplesummary}
\end{table*}

 \subsection{Favorite-Envyfree-Committee (FEC)} 
 Each population deserves their top-ranked candidate to be selected in the winning committee. However, selecting a \DiRe committee may result into an imbalance in the position of the most-favorite candidate selected from each population's ranking. A natural relaxation of FEC is finding a committee with a bounded level of envy. Specifically, in the relaxation of FEC up to $x$ where $x \in [k]$, rather than selecting the most preferred candidate, we allow for one of the top-$(x+1)$ candidates to be selected. Note that when $x=0$, FEC and FEC up to 0 are equivalent.
%All proofs are included in the Appendix.


Note that the relaxation, FEC up to $x$ is useful when a FEC does not exist. If a FEC exists, then FEC up to $x$ exists for all non-negative $x$. 


 \subsection{Utility-Envyfree-Committee (UEC)} 
%Each population deserves to minimize the difference between the utilities each one gets from the selected winning committee, where the utility is the sum of Borda scores that the population gives to the candidates in the winning committee. However, a \DiRe committee may result in an unequal utility amongst all the populations. Formally, for each $P \in \mathcal{P}$, the utility that the population gets from a winning \DiRe committee $W$ is:
%     \[ \U_P = \sum_{c \in  W} \mathtt{f}_{\Borda}^{W_P}(c) \]
% where $\mathtt{f}_{Borda}^{W_P}(c)$ is the Borda score that candidate $c$ gets based on its rank in population $P$'s winning committee $W_P$. Overall, a UEC is a $k$-sized committee such that it aims to

% % \[ \minimize_{\forall P, P' \in \mathcal{P} : P \neq P'} \max(|\U_P - \U_{P'}|) \]
% % \[ \forall P, P' \in \mathcal{P} : P \neq P', \max(|\U_P - \U_{P'}|) = 0 \]
% \[ \forall P, P' \in \mathcal{P} : P \neq P', |\U_P - \U_{P'}| = 0 \]

% %\vspace{0.2cm}

% A natural relaxation of UEC is UEC up to $\eta$ where $\eta \in \mathbb{Z}: \eta \in [0,$ $\frac{(m-1)\cdot(m)}{2}]$. This is to say that each population deserves to minimize the difference between utilities from the selected winning committee but up to $\eta$. Hence, a UEC  up to $\eta$ is a $k$-sized committee such that it ensures

% % \[ \minimize_{\forall P, P' \in \mathcal{P} : P \neq P'} \max(|\U_P - \U_{P'}|, \eta) \]
% % \[ \forall P, P' \in \mathcal{P} : P \neq P', \max(|\U_P - \U_{P'}|) \leq \eta \]
% \[ \forall P, P' \in \mathcal{P} : P \neq P', |\U_P - \U_{P'}| \leq \eta \]
% %\vspace{0.1cm}
Each population deserves to minimize the difference between the utilities each one gets from the selected winning committee, where the utility is the sum of Borda scores that the population gives to the candidates in the winning committee. However, a \DiRe committee may result into an unequal utility amongst all the populations. Formally, for each $P \in \mathcal{P}$, the utility that the population gets from a winning \DiRe committee $W$ is:
    \begin{equation} \U_P = \sum_{c \in  W} \mathtt{f}_{\Borda}^{W_P}(c) \end{equation}
where $\mathtt{f}_{Borda}^{W_P}(c)$ is the Borda score that candidate $c$ gets based on its rank in population $P$'s winning committee $W_P$. Overall, a UEC is a $k$-sized committee such that it aims to

% \[ \minimize_{\forall P, P' \in \mathcal{P} : P \neq P'} \max(|\U_P - \U_{P'}|) \]
% \[ \forall P, P' \in \mathcal{P} : P \neq P', \max(|\U_P - \U_{P'}|) = 0 \]
\begin{equation} \forall P, P' \in \mathcal{P} : P \neq P', |\U_P - \U_{P'}| = 0 \end{equation}

%\vspace{0.2cm}

A natural relaxation of UEC is UEC up to $\eta$ where $\eta \in \mathbb{Z}: \eta \in [0,$ $\frac{(m-1)\cdot(m)}{2}]$. This is to say that each population deserves to minimize the difference between utilities from the selected winning committee but up to $\eta$. Hence, a UEC  up to $\eta$ is a $k$-sized committee such that it aims to

% \[ \minimize_{\forall P, P' \in \mathcal{P} : P \neq P'} \max(|\U_P - \U_{P'}|, \eta) \]
% \[ \forall P, P' \in \mathcal{P} : P \neq P', \max(|\U_P - \U_{P'}|) \leq \eta \]
\begin{equation} \forall P, P' \in \mathcal{P} : P \neq P', |\U_P - \U_{P'}| \leq \eta \end{equation}
%\vspace{0.1cm}



Note that in line with FEC, the relaxation, UEC up to $\eta$ is useful when a UEC does not exist. If a committee $W$ is UEC, then it implies that $W$ is UEC up to $\eta$ for all $\eta$ in $[0,$ $\frac{(m-1)\cdot(m)}{2}]$. The relation does not hold the other way, which is to say that if a committee $W$ is UEC up to $\eta$, then it may not be UEC up to $\eta-1$.




% Each population deserves to minimize the difference between the weighted utilities they get from the selected winning committee. The weighted utility is the sum of Borda scores that the population gives to the candidates in the winning committee who are among their top-$k$ candidates over the maximum Borda score that they can give to candidates based on their representation constraint. Formally, for each $P \in \mathcal{P}$, the weighted utility that the population having representation constraint $l_P^R$ gets from a winning \DiRe committee $W$ is:
%     \[ \WU_P = \frac{\sum_{c \in W_P \cap W} \mathtt{f}_{\Borda}^{W_P}(c)}{\sum_{i=1}^{l_P^R}m-i} \]

% Overall, a WEC is a $k$-sized committee such that it aims to

% %\[ \minimize_{\forall P, P' \in \mathcal{P} : P \neq P'} \max(|\WU_P - \WU_{P'}|) \]
% \[ \forall P, P' \in \mathcal{P} : P \neq P', |\WU_P - \WU_{P'}| = 0 \]


% %\vspace{0.1cm}


% A natural relaxation of WEC is WEC up to $\zeta$ where $\zeta \in \mathbb{Q}: \zeta \in [0,$ $1]$. This is to say that each population deserves to minimize the difference between weighted utilities from the selected winning committee but up to $\zeta$. Hence, a WEC  up to $\zeta$ is a $k$-sized committee such that it ensures

% % \[ \minimize_{\forall P, P' \in \mathcal{P} : P \neq P'} \max(|\WU_P - \WU_{P'}|, \zeta) \]
% \[ \forall P, P' \in \mathcal{P} : P \neq P', |\WU_P - \WU_{P'}| \leq \zeta \]

\subsection{Weighted-Envyfree-Committee (WEC)} Each population deserves to minimize the difference between the weighted utilities they get from the selected winning committee. The weighted utility is the sum of Borda scores that the population gives to the candidates in the winning committee who are among their top-$k$ candidates over the maximum Borda score that they can give to candidates based on their representation constraint. Formally, for each $P \in \mathcal{P}$, the weighted utility that the population having representation constraint $l_P^R$ gets from a winning \DiRe committee $W$ is:
    \begin{equation} \WU_P = \frac{\sum_{c \in W_P \cap W} \mathtt{f}_{\Borda}^{W_P}(c)}{\sum_{i=1}^{l_P^R}m-i} \end{equation}




Overall, a WEC is a $k$-sized committee such that it aims to

%\[ \minimize_{\forall P, P' \in \mathcal{P} : P \neq P'} \max(|\WU_P - \WU_{P'}|) \]
\begin{equation} \forall P, P' \in \mathcal{P} : P \neq P', |\WU_P - \WU_{P'}| = 0 \end{equation}

\begin{example}
\label{eg-WECcalc}
The highest-scoring \DiRe committee selected in Example~\ref{eg-dire} was $W'=\{c_1, c_6, c_3, c_8\}$ ($\mathtt{f}(W')=286$). The $\WU_{IL}$ will be calculated as follows: Given, $l_{IL}^R$=2, $W_P \cap W = \{c_6, c_8\}$.

\[\WU_{IL} = \frac{\mathtt{f}_{\Borda}^{W_{IL}}(c_6) + \mathtt{f}_{\Borda}^{W_{IL}}(c_8)}{7+6} = \frac{6+4}{7+6}=\frac{10}{13}\]

Similarly, $\WU_{CA}$ will be calculated as follows: Given, $l_{CA}^R$=2, $W_P \cap W = \{c_1, c_3\}$.

\[\WU_{CA} = \frac{\mathtt{f}_{\Borda}^{W_{CA}}(c_1) + \mathtt{f}_{\Borda}^{W_{CA}}(c_3)}{7+6} = \frac{7+5}{7+6}=\frac{12}{13}\]
\end{example}
%\vspace{0.1cm}


A natural relaxation of WEC is WEC up to $\zeta$ where $\zeta \in \mathbb{Q}$ such that $\zeta \in [0,$ $1]$. This is to say that each population deserves to minimize the difference between weighted utilities from the selected winning committee but up to $\zeta$. Hence, a WEC  up to $\zeta$ is a $k$-sized committee such that it aims to

% \[ \minimize_{\forall P, P' \in \mathcal{P} : P \neq P'} \max(|\WU_P - \WU_{P'}|, \zeta) \]
\begin{equation} \forall P, P' \in \mathcal{P} : P \neq P', |\WU_P - \WU_{P'}| \leq \zeta \end{equation}


%Observe that the FEC and the UEC committee ($\{c_1, c_5, c_3, c_8\}$) selected in Example~\ref{eg-FEC} and Example~\ref{eg-UEC} is not WEC as $\WU_{IL} = \frac{11}{13}$ and $\WU_{CA}=\frac{12}{13}$.






==> new_tex/tractable.tex <==
\section{Tractable Cases}
\label{sec:tractable}



\subsection{$|\mathcal{P}|$ is small}

\subsection{$|\mathcal{G}|$ is small}

\subsection{$|\mathcal{G}|$ and $|\mathcal{P}|$ are small}


% Example 1: Conference committee election. The candidate attribute cardinality and the voter attribute cardinality are expected to be small. Hence, we can parameterize by both of these cardinalities. Hence, we get a new theorem: 

% If ∀μ ∈ Z : μ ≥ 1 and ∀π ∈ Z : π ≥ 1, then (μ, π)-DRCF problem w.r.t. |G| and |P| is solvable in polynomial time when lGD=1 ∀G∈G and lPR =1 ∀P ∈P.




% Example 2: Any example from participatory budgeting [Hershkowitz et al]. Even though undesirable, the candidates may not have attributes due to the existing election design. However, the voter attribute cardinality is expected to be small. Hence, we can parameterize by this cardinality. Hence, we get a new theorem: 

% If ∀π ∈ Z : π ≥ 1, then (μ, π)-DRCF problem w.r.t. |P| is solvable in polynomial time when lPR =1 ∀P ∈P.




% Example 3: We can pick any example from Bredereck et al or Celis et al. The voters do not have attributes. Candidates have attributes with low cardinality, which can be the parameter. Hence, we get a new theorem: 

% If ∀μ ∈ Z : μ ≥ 3, then (μ, π)-DRCF problem w.r.t. |G| is solvable in polynomial time when lGD=1 ∀G∈G.

% I plan to make the theorem statements more precise (e.g., include exact time complexity) once I formally write down the proofs. 

